3D GAN Inversion with Pose Optimization

With the recent advances in NeRF-based 3D aware GANs quality, projecting an image into the latent space of these 3D-aware GANs has a natural advantage over 2D GAN inversion: not only does it allow multi-view consistent editing of the projected image, but it also enables 3D reconstruction and novel view synthesis when given only a single image. However, the explicit viewpoint control acts as a main hindrance in the 3D GAN inversion process, as both camera pose and latent code have to be optimized simultaneously to reconstruct the given image. Most works that explore the latent space of the 3D-aware GANs rely on ground-truth camera viewpoint or deformable 3D model, thus limiting their applicability. In this work, we introduce a generalizable 3D GAN inversion method that infers camera viewpoint and latent code simultaneously to enable multi-view consistent semantic image editing. The key to our approach is to leverage pre-trained estimators for better initialization and utilize the pixel-wise depth calculated from NeRF parameters to better reconstruct the given image. We conduct extensive experiments on image reconstruction and editing both quantitatively and qualitatively, and further compare our results with 2D GAN-based editing to demonstrate the advantages of utilizing the latent space of 3D GANs. Additional results and visualizations are available at https://3dgan-inversion.github.io .

==> Figures/Inversion_method.tex <==
\begin{figure}[!t]
\centering
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\setlength{\tabcolsep}{0.2pt}
\renewcommand{\arraystretch}{0.1}
\begin{tabular}{M{0.20\linewidth} | M{0.16\linewidth}M{0.16\linewidth}M{0.16\linewidth}M{0.16\linewidth}M{0.16\linewidth}}
\backslashbox{Pose}{iters} & 0 & 150 & 300 & tuned & target \\ \\ 
\midrule
Only e4e & 
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/w_0.png}\hfill &
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/w_150.png}\hfill &
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/w_300.png}\hfill &
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/w_tuned.png}\hfill &
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/005664_real.png}\hfill\\

Only pose estimator & 
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/pose_0.png}\hfill &
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/pose_150.png}\hfill & 
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/pose_300.png}\hfill &
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/pose_tuned.png}\hfill &
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/005664_real.png}\hfill\\

Both & 
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/posew_0.png}\hfill &
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/posew_150.png}\hfill &
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/posew_300.png}\hfill &
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/wpose_tuned.png}\hfill &
\includegraphics[width=\linewidth]{Fig:ablation/Fig8/005664_real.png}\hfill &\\

\end{tabular}


\caption{Comparison of using different methods for latent vector inversion and camera pose estimation}
\label{fig:inversion_method}
\end{figure}

==> Figures/teaser.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=.44\textwidth]{Figures/KwangrokSpace/Why3D.png}\hfill\\
\caption{\textbf{Why 3D GAN is difficult to optimize?} This figure shows why 3D GAN is difficult to optimize.}
\label{fig:overall}
\end{figure}

\begin{figure}
\centering
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.1}
\begin{tabular}{M{0.2\linewidth}M{0.04\linewidth}M{0.7\linewidth}}
\multirow{3}{*}{
\makecell{
\vspace{-1pt} \\
\includegraphics[width=\linewidth]{example-images/example0.png}}
}
& \rotatebox[origin=cl]{90}{\small{age}} &
\includegraphics[width=0.19\linewidth]{example-images/example1.png}\hfill
\includegraphics[width=0.19\linewidth]{example-images/example2.png}\hfill
\includegraphics[trim=300 50 300 50,clip,width=0.19\linewidth]{example-images/example3.png}\hfill
\includegraphics[width=0.19\linewidth]{example-images/example4.png}\hfill
\includegraphics[width=0.19\linewidth]{example-images/example5.png}\hfill \\
&\rotatebox[origin=cl]{90}{\small{smile  }}&
\includegraphics[width=0.19\linewidth]{example-images/example1.png}\hfill
\includegraphics[width=0.19\linewidth]{example-images/example2.png}\hfill
\includegraphics[trim=300 50 300 50,clip,width=0.19\linewidth]{example-images/example3.png}\hfill
\includegraphics[width=0.19\linewidth]{example-images/example4.png}\hfill
\includegraphics[width=0.19\linewidth]{example-images/example5.png}\hfill \\
&\rotatebox[origin=cl]{90}{\small{gender  }}&
\includegraphics[width=0.19\linewidth]{example-images/example1.png}\hfill
\includegraphics[width=0.19\linewidth]{example-images/example2.png}\hfill
\includegraphics[trim=300 50 300 50,clip,width=0.19\linewidth]{example-images/example3.png}\hfill
\includegraphics[width=0.19\linewidth]{example-images/example4.png}\hfill
\includegraphics[width=0.19\linewidth]{example-images/example5.png}\hfill \\


\end{tabular}
    \caption{3D reconstruction and latent-based editing ability with our method.}
    \label{fig:my_label}
\end{figure}


% \begin{figure}
% % \includegraphics[width=0.2\linewidth]{example-images/example0.png}
% \centering
% \small

% \newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
% \setlength{\tabcolsep}{1pt}
% \renewcommand{\arraystretch}{0.1}
% \begin{tabular}{M{0.05\linewidth}M{0.7\linewidth}}
%  \rotatebox[origin=cl]{90}{age} &
% \includegraphics[width=0.19\linewidth]{example-images/example1.png}\hfill
% \includegraphics[width=0.19\linewidth]{example-images/example2.png}\hfill
% \includegraphics[trim=300 50 300 50,clip,width=0.19\linewidth]{example-images/example3.png}\hfill
% \includegraphics[width=0.19\linewidth]{example-images/example4.png}\hfill
% \includegraphics[width=0.19\linewidth]{example-images/example5.png}\hfill \\
% \rotatebox[origin=cl]{90}{smile}&
% \includegraphics[width=0.19\linewidth]{example-images/example1.png}\hfill
% \includegraphics[width=0.19\linewidth]{example-images/example2.png}\hfill
% \includegraphics[trim=300 50 300 50,clip,width=0.19\linewidth]{example-images/example3.png}\hfill
% \includegraphics[width=0.19\linewidth]{example-images/example4.png}\hfill
% \includegraphics[width=0.19\linewidth]{example-images/example5.png}\hfill \\
% \rotatebox[origin=cl]{90}{gender }&
% \includegraphics[width=0.19\linewidth]{example-images/example1.png}\hfill
% \includegraphics[width=0.19\linewidth]{example-images/example2.png}\hfill
% \includegraphics[trim=300 50 300 50,clip,width=0.19\linewidth]{example-images/example3.png}\hfill
% \includegraphics[width=0.19\linewidth]{example-images/example4.png}\hfill
% \includegraphics[width=0.19\linewidth]{example-images/example5.png}\hfill \\


% \end{tabular}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

==> Figures/vs2D.tex <==
\begin{figure}[!t]
\centering
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{M{0.15\linewidth} M{0.05\linewidth} M{0.15\linewidth} M{0.15\linewidth} M{0.15\linewidth} M{0.15\linewidth} M{0.15\linewidth}}
\multirow{2}{*}{
\makecell{
% \vspace{-1pt} \\
\includegraphics[width=\linewidth]{Fig:vs2D/camera_manipulation/002292.png}}
}
& \rotatebox[origin=rl]{90}{\small{2D}} &
\includegraphics[width=\linewidth]{Fig:vs2D/camera_manipulation/002292_2D_sample0.png}\hfill &
\includegraphics[width=\linewidth]{Fig:vs2D/camera_manipulation/002292_2D_sample1.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera_manipulation/002292_2D_sample2.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera_manipulation/002292_2D_sample3.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera_manipulation/002292_2D_sample4.png}\hfill \\
&\rotatebox[origin=rl]{90}{\small{3D}}&
\includegraphics[width=\linewidth]{Fig:vs2D/camera_manipulation/002292_3D_0.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera_manipulation/002292_3D_1.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera_manipulation/002292_3D_2.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera_manipulation/002292_3D_3.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera_manipulation/002292_3D_4.png}\hfill \\

%trim=300 50 300 50,clip,
\end{tabular}


\caption{\textbf{Comparison of pose manipulation of real images inverted with 2D GANs and 3D GANs.} As can be seen, pose manipulation using PTI on StyleGAN2 (first row) only allows for implicit control by the editing magnitude and larger step sizes result in undesired transformations. On the other hand, using our method on EG3D (second row), allows for explicit control and because the acquired latent representation are viewpoint independent, the edits geometrically consistent.}
\label{fig:pose_manipulation_2d}
% \end{figure}

% \begin{figure}[!t]
\centering
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\setlength{\tabcolsep}{0.2pt}
\renewcommand{\arraystretch}{0.1}
\begin{tabular}{M{0.15\linewidth} M{0.05\linewidth} M{0.15\linewidth} M{0.15\linewidth} M{0.15\linewidth} M{0.15\linewidth} M{0.15\linewidth}}
\multirow{2}{*}{
\makecell{
% \vspace{-1pt} \\
\includegraphics[width=\linewidth]{Fig:vs2D/camera+att/001663.png}}
}
& \rotatebox[origin=rl]{90}{\small{2D}} &
\includegraphics[width=\linewidth]{Fig:vs2D/camera+att/001663_2D_sample0.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera+att/001663_2D_sample1.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera+att/001663_2D_sample2.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera+att/001663_2D_sample3.png}\hfill &
\includegraphics[width=\linewidth]{Fig:vs2D/camera+att/001663_2D_sample4.png}\hfill \\ 
&\rotatebox[origin=rl]{90}{\small{3D}}&
\includegraphics[width=\linewidth]{Fig:vs2D/camera+att/001663_3D_0.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera+att/001663_3D_1.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera+att/001663_3D_2.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera+att/001663_3D_3.png}\hfill&
\includegraphics[width=\linewidth]{Fig:vs2D/camera+att/001663_3D_4.png}\hfill \\
\end{tabular}


\caption{\textbf{Simultaneous attribute editing and viewpoint shift comparison with StyleGAN2}}
\label{fig:my_label}
\end{figure}

==> Tables/algorithm.tex <==
\begin{algorithm}[!t]
% \small
\SetAlgoLined
 \KwIn{real image $x$; canonical pose $\pi_c$; gradient-based optimizer $F'$; depth smoothness regularizer $DR$; depth based reprojection $proj()$; camera intrinsics $K$ }
 \KwOut{the reconstructed image $\hat{y}$}
 Initialize() the code and pose $(w, \pi)$ = $(w', \pi ')$\;
 \While{not converged}{
  $Loss \leftarrow L\left(x, \mathcal{G}^\mathrm{c}_\mathrm{3D}(\mathbf{w}, \pi; \theta)\right)$\;
  $w \leftarrow w - \eta F'(\nabla_w Loss)$\;
  $\mathrm{projected} \leftarrow \mathcal{G}^\mathrm{c}_\mathrm{3D}(\mathbf{w}, \pi; \theta) \langle proj(\mathcal{G}^\mathrm{d}_\mathrm{3D}(\mathbf{w}, \pi; \theta), \pi,K)\rangle $ \;
  $Loss \leftarrow L\left(\mathcal{G}^\mathrm{c}_\mathrm{3D}(\mathbf{w}, \pi; \theta)),\mathrm{projected},\right)$\;
  $\pi \leftarrow \pi - \eta F'(\nabla_\pi Loss)$\;
  
 }
%   \If{pivotal tuning}{
\While{not converged}{
$Loss \leftarrow L\left(x,  \mathcal{G}^\mathrm{c}_\mathrm{3D}(\mathbf{w}, \pi; \theta))\right) + DR(\mathcal{G}^\mathrm{d}_\mathrm{3D}(\mathbf{w}, \pi; \theta))       $\;
$\theta \leftarrow \theta - \eta F'(\nabla_\theta Loss)$\;
}
%   }
%  \STATE
%  $Loss \leftarrow L\left(x, \mathcal{R}(\pi^*, G(\mathbf{w}; \theta))\right)$\;
%  $\theta \leftarrow \theta - \eta F'(\nabla_\theta L)$\;
%  }
$\hat{y}\leftarrow \mathcal{G}^\mathrm{c}_\mathrm{3D}(\mathbf{w}, \pi; \theta)$
  \caption{Proposed method.}
 \label{alg:method}
\end{algorithm}

==> Tables/baseline_alg.tex <==
% \begin{basealgorithm}[!t]
% \SetAlgoLined
% \begin{footnotesize}
%     % \PyComment{Stage 1: pre-training matching networks} \\
%     % \PyCode{\rc{for} I\_S, I\_T, GT\_keypoints \rc{in} loader:} \\

%     \PyCode{\rc{for} I\_S, I\_T, GT\_keypoints \rc{in} loader:} \\
%         \Indp
%         \PyCode{pred\_map = argmax(confmatch.net(I\_S, I\_T))} \\
%         \PyCode{pred\_flow = convert\_flow(pred\_map)} \\
%         \PyCode{GT\_flow = keypoint\_to\_flow(GT\_keypoints)} \\
%         \PyCode{loss\_matching\_sup = EPE(pred\_flow, GT\_flow)} \\
%         \PyCode{Loss.backward(); update(confmatch.net)} \\
%         \Indm
% \end{footnotesize}

% \caption{GT camera pose during optimization.}
% \label{algo:baseline1}
% \end{basealgorithm}
% \begin{basealgorithm}[!t]
% \SetAlgoLined
% \begin{footnotesize}
%     % \PyComment{Stage 1: pre-training matching networks} \\
%     % \PyCode{\rc{for} I\_S, I\_T, GT\_keypoints \rc{in} loader:} \\

%     \PyCode{\rc{for} I\_S, I\_T, GT\_keypoints \rc{in} loader:} \\
%         \Indp
%         \PyCode{pred\_map = argmax(confmatch.net(I\_S, I\_T))} \\
%         \PyCode{pred\_flow = convert\_flow(pred\_map)} \\
%         \PyCode{GT\_flow = keypoint\_to\_flow(GT\_keypoints)} \\
%         \PyCode{loss\_matching\_sup = EPE(pred\_flow, GT\_flow)} \\
%         \PyCode{Loss.backward(); update(confmatch.net)} \\
%         \Indm
% \end{footnotesize}

% \caption{Gradient descent to optimize camera.}
% \label{algo:baseline2}
% \end{basealgorithm}

\begin{basealgorithm}[!t]
% \small
\SetAlgoLined
 \KwIn{real image $x$ from viewpoint $\pi^*$; a pre-trained generator $\mathcal{R}(\cdot, G(\cdot;\theta))$; gradient-based optimizer $F'$.}
 \KwOut{the latent code $w$}
 Initialize() the code $w$ = $w'$\;
 \While{not converged}{
  $Loss \leftarrow L\left(x, \mathcal{G}^\mathrm{c}_\mathrm{3D}(\mathbf{w}, \pi^*; \theta)\right)$\;
  $w \leftarrow w - \eta F'(\nabla_w L)$\;
 }
  \If{pivotal tuning}{
        \While{not converged}{
         $Loss \leftarrow L\left(x, \mathcal{G}^\mathrm{c}_\mathrm{3D}(\mathbf{w}, \pi^*; \theta)\right)$\;
        $\theta \leftarrow \theta - \eta F'(\nabla_\theta L)$\;
        }
  }
%  \STATE
%  $Loss \leftarrow L\left(x, \mathcal{R}(\pi^*, G(w; \theta))\right)$\;
%  $\theta \leftarrow \theta - \eta F'(\nabla_\theta L)$\;
%  }
  \caption{GT camera pose during optimization.}
 \label{alg:baseline1}
\end{basealgorithm}

\begin{basealgorithm}[!t]
% \small
\SetAlgoLined
 \KwIn{real image $x$; a pre-trained generator $\mathcal{R}(\cdot, G(\cdot;\theta))$; gradient-based optimizer $F'$.}
 \KwOut{the latent code $w$}
 Initialize() the code and pose $(w, \pi)$ = $(w', \pi ')$\;
 \While{not converged}{
  $Loss \leftarrow L\left(x, \mathcal{G}^\mathrm{c}_\mathrm{3D}(\mathbf{w}, \pi; \theta)\right)$\;
  $(w, \pi) \leftarrow (w, \pi) - \eta F'(\nabla_{w, \pi} L)$\;
 }
  \If{pivotal tuning}{
        \While{not converged}{
        $Loss \leftarrow L\left(x,\mathcal{G}^\mathrm{c}_\mathrm{3D}(\mathbf{w}, \pi; \theta)\right)$\;
        $\theta \leftarrow \theta - \eta F'(\nabla_\theta L)$\;
        }
  }
%  \STATE
%  $Loss \leftarrow L\left(x, \mathcal{R}(\pi^*, G(w; \theta))\right)$\;
%  $\theta \leftarrow \theta - \eta F'(\nabla_\theta L)$\;
%  }
  \caption{Gradient descent to optimize camera.}
 \label{alg:baseline2}
\end{basealgorithm}

==> Tables/edit_results.tex <==
\begin{table}[!t]
\small
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
% \setlength{\tabcolsep}{0.2pt}
% \renewcommand{\arraystretch}{0.1}

\begin{subtable}[h]{\linewidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{M{0.05\linewidth} |M{0.08\linewidth}|  M{0.1\linewidth} M{0.1\linewidth}M{0.1\linewidth} M{0.1\linewidth} M{0.1\linewidth} M{0.1\linewidth} M{0.1\linewidth} }
\toprule
Attr. & $\gamma$ & SG2 & SG2 $\mathcal{W}+$ & PTI & SG2$^\dagger$ & SG2$^\dagger$ $\mathcal{W}+$ & PTI$^\dagger$ & Ours \\
\midrule
\multirow{7}{*}{
\rotatebox[origin=c]{90}{Age}
}
&-3.6&	-7.320&	-6.598&	-6.625&	-6.522&	-6.228&	-6.831&	-7.146 \\
&-2.4&	-5.455&	-4.804&	-4.526&	-4.834&	-4.518&	-4.726&	-4.922\\
&-1.2&	-3.02&	-2.557&	-2.3&	-2.737&	-2.476&	-2.518&	-2.584\\
&0&	0&	0&	0&	0&	0&	0&	0\\
&1.2&	3.142&	2.696&	2.656&	3.141&	3.075&	2.570&	2.725\\
&2.4&	6.464&	5.74&	5.506&	6.686&	6.414&	5.574&	5.929\\
&3.6&	9.868&	8.926&	8.558&	10.267&	10.077&	8.668&	9.296\\

\midrule
\multirow{7}{*}{
\rotatebox[origin=c]{90}{Smile}
}
&-2&	-3.150&	-2.392&	-2.715&	-2.627&	-2.111&	-2.107&	-2.711\\
&-1.33&	-2.210&	-1.597&	-1.838&	-1.829&	-1.501&	-1.447&	-1.882\\
&-0.67&	-1.129&	-0.798&	-0.920&	-0.940&	-0.764&	-0.714&	-0.937\\
&0&	0&	0&	0&	0&	0&	0&	0\\
&0.66&	0.964&	0.817&	0.850&	0.831&	0.711&	0.608&	0.919\\
&1.33&	1.925&	1.583&	1.734&	1.558&	1.271&	1.364&	1.854\\
&2&	2.762&	2.226&	2.524&	2.189&	1.861&	1.962&	2.694\\
\bottomrule
\end{tabular}}
\caption{Quantitative evaluation of manipulation capability}
\label{tab:magnipulation_capability}
\end{subtable}
\hfill
\begin{subtable}[h]{\linewidth}
\centering
% \includegraphics[width=\linewidth]{fig: edit/Chart.pdf}\hfill 
\resizebox{\linewidth}{!}{
% \begin{tikzpicture}
%     \begin{axis}[
%         xlabel=$x$,
%         ylabel=$y$,
%         xmin=0, xmax=4,
%         ymin=0, ymax=16,
%         xtick={1,2,3},
%         ytick={3, 5, 10, 15}
%         ]
%     \addplot[smooth,color=orange,mark=x] plot coordinates {
%         (1,4)
%         (2,3)
%         (3,1)
%     };
% \addlegendentry{Rendering Loss}

%     \addplot[smooth,color=blue,mark=x] plot coordinates {
%             (1, 14)
%             (2, 10)
%             (3, 5)
%         };
% \addlegendentry{Camera Loss}
% \end{axis}
% \end{tikzpicture} 
% Magnitude	SG2	SG2W+	PTI	SG2†	SG2†W+	PTI†	Ours
\begin{tikzpicture}[scale=1]
 \pgfplotsset{grid style={dashed,gray}}
\begin{axis}[name=ax1, minor tick num=1,
legend style={font=\small, at={(-0.1,0.-0.2)},anchor=north west,legend columns=2},
ymajorgrids=true,
xlabel={\normalsize{Age Magnitude ($\gamma$)}},
ylabel={\normalsize{Identity Similarity}}
]
\addlegendentry{SG2}
\addplot [red,ultra thick] table [x={Magnitude}, y={SG2}] {tab:similarity_data/age_similarity.dat};
\addlegendentry{SG2 $\mathcal{W}+$}
\addplot [orange,ultra thick] table [x={Magnitude}, y={SG2W+}] {tab:similarity_data/age_similarity.dat};
\addlegendentry{PTI}
\addplot [pink,ultra thick] table [x={Magnitude}, y={PTI}] {tab:similarity_data/age_similarity.dat};
\addlegendentry{SG2$^\dagger$}
\addplot [lime,ultra thick] table [x={Magnitude}, y={SG2†}] {tab:similarity_data/age_similarity.dat};
\addlegendentry{SG2$^\dagger$ $\mathcal{W}+$}
\addplot [olive,ultra thick] table [x={Magnitude}, y={SG2†W+}] {tab:similarity_data/age_similarity.dat};
\addlegendentry{PTI$^\dagger$}
\addplot [green,ultra thick] table [x={Magnitude}, y={PTI†}] {tab:similarity_data/age_similarity.dat};
\addlegendentry{Ours}
\addplot [blue,ultra thick] table [x={Magnitude}, y={Ours}] {tab:similarity_data/age_similarity.dat};
\legend{}
\end{axis}
\begin{axis}[ at={(ax1.south east)}, minor tick num=1, xshift=10pt,
legend style={draw=none, font=\normalsize, at={(0.8, 1)}, anchor=south east, legend columns=7},
yticklabels={,,}, ymajorgrids=true,
xlabel={\normalsize{Smile Magnitude ($\gamma$)}}]
\addlegendentry{SG2}
\addplot [red,ultra thick] table [x={Magnitude}, y={SG2}] {tab:similarity_data/smile_similarity.dat};
\addlegendentry{SG2 $\mathcal{W}+$}
\addplot [orange,ultra thick] table [x={Magnitude}, y={SG2W+}] {tab:similarity_data/smile_similarity.dat};
\addlegendentry{PTI}
\addplot [pink,ultra thick] table [x={Magnitude}, y={PTI}] {tab:similarity_data/smile_similarity.dat};
\addlegendentry{SG2$^\dagger$}
\addplot [lime,ultra thick] table [x={Magnitude}, y={SG2†}] {tab:similarity_data/smile_similarity.dat};
\addlegendentry{SG2$^\dagger$ $\mathcal{W}+$}
\addplot [olive,ultra thick] table [x={Magnitude}, y={SG2†W+}] {tab:similarity_data/smile_similarity.dat};
\addlegendentry{PTI$^\dagger$}
\addplot [green,ultra thick] table [x={Magnitude}, y={PTI†}] {tab:similarity_data/smile_similarity.dat};
\addlegendentry{Ours}
\addplot [blue,ultra thick] table [x={Magnitude}, y={Ours}] {tab:similarity_data/smile_similarity.dat};
\end{axis}
\end{tikzpicture}
}
\caption{Quantitative evaluation of identity preservation}
\label{tab:edit_similarity}
\end{subtable}
\hfill
\caption{\textbf{Quantitative evaluation of editability.} In (a), we apply varying magnitudes $\gamma$ of age edit and smile edit to the latent codes acquired by each method and measure the amount of age change and difference of smile extent respectively. In (b), we also compare the identity similarity between the original image and edited images.}
\label{tab:temps}
\end{table}


